Temporally coherent video anonymization through GAN inpainting

This work tackles the problem of temporally coherent face anonymization in natural video streams.We propose JaGAN, a two-stage system starting with detecting and masking out faces with black image patches in all individual frames of the video. The second stage leverages a privacy-preserving Video Generative Adversarial Network designed to inpaint the missing image patches with artificially generated faces. Our initial experiments reveal that image based generative models are not capable of inpainting patches showing temporal coherent appearance across neighboring video frames. To address this issue we introduce a newly curated video collection, which is made publicly available for the research community along with this paper. We also introduce the Identity Invariance Score IdI as a means to quantify temporal coherency between neighboring frames.

==> egbib_backup.tex <==
% Encoding: UTF-8

@misc{eu-32016R0679,
  author={{Council of European Union}},
  title={General Data Protection Regulation ({EU}) no 2016/679},
  year={2016},
  note={\url{http://data.europa.eu/eli/reg/2016/679/oj}},
}

@incollection{NIPS2014_5423,
title = {Generative Adversarial Nets},
author = {Goodfellow, Ian and Pouget-Abadie, Jean and Mirza, Mehdi and Xu, Bing and Warde-Farley, David and Ozair, Sherjil and Courville, Aaron and Bengio, Yoshua},
booktitle = {Advances in Neural Information Processing Systems 27},
editor = {Z. Ghahramani and M. Welling and C. Cortes and N. D. Lawrence and K. Q. Weinberger},
pages = {2672--2680},
year = {2014},
publisher = {Curran Associates, Inc.}
}

@inproceedings{DBLP:conf/iclr/KarrasALL18,
  author    = {Tero Karras and
               Timo Aila and
               Samuli Laine and
               Jaakko Lehtinen},
  title     = {Progressive Growing of GANs for Improved Quality, Stability, and Variation},
  booktitle = {6th International Conference on Learning Representations, {ICLR} 2018,
               Vancouver, BC, Canada, April 30 - May 3, 2018, Conference Track Proceedings},
  publisher = {OpenReview.net},
  year      = {2018},
  timestamp = {Thu, 04 Apr 2019 13:20:09 +0200},
}



@inproceedings{DBLP:conf/eccv/FengWSWZ18,
  author    = {Yao Feng and
               Fan Wu and
               Xiaohu Shao and
               Yanfeng Wang and
               Xi Zhou},
  editor    = {Vittorio Ferrari and
               Martial Hebert and
               Cristian Sminchisescu and
               Yair Weiss},
  title     = {Joint 3D Face Reconstruction and Dense Alignment with Position Map
               Regression Network},
  booktitle = {Computer Vision - {ECCV} 2018 - 15th European Conference, Munich,
               Germany, September 8-14, 2018, Proceedings, Part {XIV}},
  series    = {Lecture Notes in Computer Science},
  volume    = {11218},
  pages     = {557--574},
  publisher = {Springer},
  year      = {2018},
  url       = {https://doi.org/10.1007/978-3-030-01264-9\_33},
  doi       = {10.1007/978-3-030-01264-9\_33},
  timestamp = {Tue, 14 May 2019 10:00:45 +0200},
  biburl    = {https://dblp.org/rec/conf/eccv/FengWSWZ18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


@inproceedings{DBLP:conf/cvpr/ZhangSQ17,
  author    = {Zhifei Zhang and
               Yang Song and
               Hairong Qi},
  title     = {Age Progression/Regression by Conditional Adversarial Autoencoder},
  booktitle = {2017 {IEEE} Conference on Computer Vision and Pattern Recognition,
               {CVPR} 2017, Honolulu, HI, USA, July 21-26, 2017},
  pages     = {4352--4360},
  publisher = {{IEEE} Computer Society},
  year      = {2017},
  url       = {https://doi.org/10.1109/CVPR.2017.463},
  doi       = {10.1109/CVPR.2017.463},
  timestamp = {Wed, 16 Oct 2019 14:14:50 +0200},
  biburl    = {https://dblp.org/rec/conf/cvpr/ZhangSQ17.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/corr/abs-1810-10220,
  author    = {Jian Li and
               Yabiao Wang and
               Changan Wang and
               Ying Tai and
               Jianjun Qian and
               Jian Yang and
               Chengjie Wang and
               Ji{-}Lin Li and
               Feiyue Huang},
  title     = {{DSFD:} Dual Shot Face Detector},
  journal   = {CoRR},
  volume    = {abs/1810.10220},
  year      = {2018},
  archivePrefix = {arXiv},
  eprint    = {1810.10220},
  timestamp = {Tue, 20 Nov 2018 12:24:39 +0100}
}



@InProceedings{DBLP:conf/eccv/FengWSWZ18,
  author    = {Yao Feng and Fan Wu and Xiaohu Shao and Yanfeng Wang and Xi Zhou},
  title     = {Joint 3D Face Reconstruction and Dense Alignment with Position Map Regression Network},
  booktitle = {Computer Vision - {ECCV} 2018 - 15th European Conference, Munich, Germany, September 8-14, 2018, Proceedings, Part {XIV}},
  year      = {2018},
  pages     = {557--574},
  crossref  = {DBLP:conf/eccv/2018-14},
  timestamp = {Tue, 14 May 2019 10:00:45 +0200}
}

@INPROCEEDINGS{8237891,
author={H. {Zhang} and T. {Xu} and H. {Li} and S. {Zhang} and X. {Wang} and X. {Huang} and D. {Metaxas}},
booktitle={2017 IEEE International Conference on Computer Vision (ICCV)},
title={StackGAN: Text to Photo-Realistic Image Synthesis with Stacked Generative Adversarial Networks},
year={2017},
volume={},
number={},
pages={5908-5916},
keywords={computer vision;feature extraction;image representation;image resolution;object recognition;realistic images;text analysis;sketch-refinement process;sketches the primitive shape;colors;given text description;low-resolution images;Stage-II GAN;Stage-I results;text descriptions;high-resolution images;photo-realistic details;synthesized images;StackGAN;photo-realistic image synthesis;stacked generative adversarial networks;existing textto- image approaches;vivid object parts;Gallium nitride;Training;Generators;Manifolds;Image resolution;Shape;Gaussian distribution},
ISSN={2380-7504},
month={Oct},}

@article{DBLP:journals/corr/ReedAYLSL16,
       author = {{Reed}, Scott and {Akata}, Zeynep and {Yan}, Xinchen and
         {Logeswaran}, Lajanugen and {Schiele}, Bernt and {Lee}, Honglak},
        title = "{Generative Adversarial Text to Image Synthesis}",
      journal = {arXiv e-prints},
     keywords = {Computer Science - Neural and Evolutionary Computing, Computer Science - Computer Vision and Pattern Recognition},
         year = 2016,
        month = may,
          eid = {arXiv:1605.05396},
        pages = {arXiv:1605.05396},
archivePrefix = {arXiv},
       eprint = {1605.05396},
 primaryClass = {cs.NE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016arXiv160505396R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@INPROCEEDINGS{8100223,
author={F. {Luan} and S. {Paris} and E. {Shechtman} and K. {Bala}},
booktitle={2017 IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
title={Deep Photo Style Transfer},
year={2017},
volume={},
number={},
pages={6997-7005},
keywords={image colour analysis;learning (artificial intelligence);neural nets;photography;photographs;reference images;photorealistic style transfer;neural network;painterly transfer;reference style;image content;photographic style transfer;deep-learning approach;deep photo style transfer;Image color analysis;Distortion;Semantics;Buildings;Image segmentation;Meteorology;Painting},
ISSN={1063-6919},
month={July},}

@inproceedings{DBLP:conf/cvpr/SchroffKP15,
  author    = {Florian Schroff and
               Dmitry Kalenichenko and
               James Philbin},
  title     = {FaceNet: {A} unified embedding for face recognition and clustering},
  booktitle = {{IEEE} Conference on Computer Vision and Pattern Recognition, {CVPR}
               2015, Boston, MA, USA, June 7-12, 2015},
  pages     = {815--823},
  year      = {2015},
  crossref  = {DBLP:conf/cvpr/2015},
  timestamp = {Thu, 25 May 2017 00:41:13 +0200}
}

@inproceedings{CycleGAN2017,
  title={Unpaired Image-to-Image Translation using Cycle-Consistent Adversarial Networks},
  author={Zhu, Jun-Yan and Park, Taesung and Isola, Phillip and Efros, Alexei A},
  booktitle={Computer Vision (ICCV), 2017 IEEE International Conference on},
  year={2017}
}

@INPROCEEDINGS{8099502,
author={C. {Ledig} and L. {Theis} and F. {Huszár} and J. {Caballero} and A. {Cunningham} and A. {Acosta} and A. {Aitken} and A. {Tejani} and J. {Totz} and Z. {Wang} and W. {Shi}},
booktitle={2017 IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
title={Photo-Realistic Single Image Super-Resolution Using a Generative Adversarial Network},
year={2017},
volume={},
number={},
pages={105-114},
keywords={feedforward neural nets;image reconstruction;image resolution;image sampling;image texture;realistic images;upscaling factors;perceptual loss function;adversarial loss;content loss;natural image manifold;discriminator network;perceptual similarity;deep residual network;photo-realistic textures;heavily downsampled images;SRGAN;high-resolution images;photo-realistic single image super-resolution;generative adversarial network;deeper convolutional neural networks;super-resolution methods;objective function;mean squared reconstruction error;signal-to-noise ratios;photo-realistic natural images;Image resolution;Signal resolution;Gallium nitride;Image reconstruction;Manifolds;Training;Network architecture},
month={July},}

@inproceedings{DBLP:conf/cvpr/Wang0ZTKC18,
  author    = {Ting{-}Chun Wang and
               Ming{-}Yu Liu and
               Jun{-}Yan Zhu and
               Andrew Tao and
               Jan Kautz and
               Bryan Catanzaro},
  title     = {High-Resolution Image Synthesis and Semantic Manipulation With Conditional
               GANs},
  booktitle = {2018 {IEEE} Conference on Computer Vision and Pattern Recognition,
               {CVPR} 2018, Salt Lake City, UT, USA, June 18-22, 2018},
  pages     = {8798--8807},
  year      = {2018},
  crossref  = {DBLP:conf/cvpr/2018},
  timestamp = {Tue, 20 Nov 2018 12:25:48 +0100},
}


@inproceedings{DBLP:conf/nips/GulrajaniAADC17,
  author    = {Ishaan Gulrajani and
               Faruk Ahmed and
               Mart{\'{\i}}n Arjovsky and
               Vincent Dumoulin and
               Aaron C. Courville},
  title     = {Improved Training of Wasserstein GANs},
  booktitle = {Advances in Neural Information Processing Systems 30: Annual Conference
               on Neural Information Processing Systems 2017, 4-9 December 2017,
               Long Beach, CA, {USA}},
  pages     = {5769--5779},
  year      = {2017},
  crossref  = {DBLP:conf/nips/2017},
  timestamp = {Mon, 27 Nov 2017 12:38:48 +0100}
}

@inproceedings{Neustaedter2003BalancingPA,
  title={Balancing Privacy and Awareness in Home Media Spaces 1},
  author={Carman Neustaedter and Saul N. Greenberg},
  year={2003}
}

@article{10.1145/330534.330540,
author = {Crowley, James L. and Coutaz, Jo\"{e}lle and B\'{e}rard, Fran\c{c}ois},
title = {Perceptual User Interfaces: Things That See},
year = {2000},
issue_date = {March 2000},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
volume = {43},
number = {3},
journal = {Commun. ACM},
month = mar,
pages = {54–ff.},
numpages = {11}
}

@inproceedings{10.1145/240080.240295,
author = {Hudson, Scott E. and Smith, Ian},
title = {Techniques for Addressing Fundamental Privacy and Disruption Tradeoffs in Awareness Support Systems},
year = {1996},
isbn = {0897917650},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
booktitle = {Proceedings of the 1996 ACM Conference on Computer Supported Cooperative Work},
pages = {248–257},
numpages = {10},
keywords = {audio, video, distributed work groups, awareness support, visualization, media spaces, privacy},
location = {Boston, Massachusetts, USA},
series = {CSCW ’96}
}

@article{DBLP:journals/corr/McPhersonSS16,
       author = {{McPherson}, Richard and {Shokri}, Reza and {Shmatikov}, Vitaly},
        title = "{Defeating Image Obfuscation with Deep Learning}",
      journal = {arXiv e-prints},
     keywords = {Computer Science - Cryptography and Security, Computer Science - Computer Vision and Pattern Recognition},
         year = 2016,
        month = sep,
          eid = {arXiv:1609.00408},
        pages = {arXiv:1609.00408},
archivePrefix = {arXiv},
       eprint = {1609.00408},
 primaryClass = {cs.CR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016arXiv160900408M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@article{Ribaric2015AnOO,
  title={An overview of face de-identification in still images and videos},
  author={Slobodan Ribaric and Nikola Pavesic},
  journal={2015 11th IEEE International Conference and Workshops on Automatic Face and Gesture Recognition (FG)},
  year={2015},
  volume={04},
  pages={1-6}
}

@inproceedings{10.1145/358916.358935,
author = {Boyle, Michael and Edwards, Christopher and Greenberg, Saul},
title = {The Effects of Filtered Video on Awareness and Privacy},
year = {2000},
isbn = {1581132220},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
booktitle = {Proceedings of the 2000 ACM Conference on Computer Supported Cooperative Work},
pages = {1–10},
numpages = {10},
keywords = {awareness, casual interaction, media spaces, distributed groupware, always-on video},
location = {Philadelphia, Pennsylvania, USA},
series = {CSCW ’00}
}

@article{10.1109/TKDE.2005.32,
author = {Newton, Elaine M. and Sweeney, Latanya and Malin, Bradley},
title = {Preserving Privacy by De-Identifying Face Images},
year = {2005},
issue_date = {February 2005},
publisher = {IEEE Educational Activities Department},
address = {USA},
volume = {17},
number = {2},
issn = {1041-4347},
journal = {IEEE Trans. on Knowl. and Data Eng.},
month = feb,
pages = {232–243},
numpages = {12},
keywords = {privacy, k-anonymity., Index Terms- Video surveillance, privacy-preserving data mining}
}



@article{DBLP:journals/corr/MirzaO14,
       author = {{Mirza}, Mehdi and {Osindero}, Simon},
        title = "{Conditional Generative Adversarial Nets}",
      journal = {arXiv e-prints},
     keywords = {Computer Science - Machine Learning, Computer Science - Artificial Intelligence, Computer Science - Computer Vision and Pattern Recognition, Statistics - Machine Learning},
         year = 2014,
        month = nov,
          eid = {arXiv:1411.1784},
        pages = {arXiv:1411.1784},
archivePrefix = {arXiv},
       eprint = {1411.1784},
 primaryClass = {cs.LG},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014arXiv1411.1784M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@InProceedings{pix2pix2016,
author = {Isola, Phillip and Zhu, Jun-Yan and Zhou, Tinghui and Efros, Alexei A.},
title = {Image-To-Image Translation With Conditional Adversarial Networks},
booktitle = {The IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
month = {July},
year = {2017}
} 

@article{DBLP:journals/corr/abs-1710-10196,
       author = {{Karras}, Tero and {Aila}, Timo and {Laine}, Samuli and
         {Lehtinen}, Jaakko},
        title = "{Progressive Growing of GANs for Improved Quality, Stability, and Variation}",
      journal = {arXiv e-prints},
     keywords = {Computer Science - Neural and Evolutionary Computing, Computer Science - Machine Learning, Statistics - Machine Learning},
         year = 2017,
        month = oct,
          eid = {arXiv:1710.10196},
        pages = {arXiv:1710.10196},
archivePrefix = {arXiv},
       eprint = {1710.10196},
 primaryClass = {cs.NE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017arXiv171010196K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



  
@inproceedings{DBLP:conf/icml/MeschederGN18,
  author    = {Lars M. Mescheder and
               Andreas Geiger and
               Sebastian Nowozin},
  title     = {Which Training Methods for GANs do actually Converge?},
  booktitle = {Proceedings of the 35th International Conference on Machine Learning,
               {ICML} 2018, Stockholmsm{\"{a}}ssan, Stockholm, Sweden, July
               10-15, 2018},
  pages     = {3478--3487},
  year      = {2018},
  crossref  = {DBLP:conf/icml/2018},
  timestamp = {Fri, 13 Jul 2018 14:58:25 +0200}
}


@inproceedings{DBLP:conf/miccai/RonnebergerFB15,
  author    = {Olaf Ronneberger and
               Philipp Fischer and
               Thomas Brox},
  title     = {U-Net: Convolutional Networks for Biomedical Image Segmentation},
  booktitle = {Medical Image Computing and Computer-Assisted Intervention - {MICCAI}
               2015 - 18th International Conference Munich, Germany, October 5 -
               9, 2015, Proceedings, Part {III}},
  pages     = {234--241},
  year      = {2015},
  crossref  = {DBLP:conf/miccai/2015-3},
  timestamp = {Tue, 23 May 2017 01:11:14 +0200},
}

@inproceedings{DBLP:conf/cvpr/Yu0YSLH18,
  author    = {Jiahui Yu and
               Zhe Lin and
               Jimei Yang and
               Xiaohui Shen and
               Xin Lu and
               Thomas S. Huang},
  title     = {Generative Image Inpainting With Contextual Attention},
  booktitle = {2018 {IEEE} Conference on Computer Vision and Pattern Recognition,
               {CVPR} 2018, Salt Lake City, UT, USA, June 18-22, 2018},
  pages     = {5505--5514},
  year      = {2018},
  crossref  = {DBLP:conf/cvpr/2018},
  timestamp = {Tue, 20 Nov 2018 12:25:48 +0100},
}



@inproceedings{DBLP:conf/nips/DentonCSF15,
  author    = {Emily L. Denton and
               Soumith Chintala and
               Arthur Szlam and
               Rob Fergus},
  title     = {Deep Generative Image Models using a Laplacian Pyramid of Adversarial
               Networks},
  booktitle = {Advances in Neural Information Processing Systems 28: Annual Conference
               on Neural Information Processing Systems 2015, December 7-12, 2015,
               Montreal, Quebec, Canada},
  pages     = {1486--1494},
  year      = {2015},
  crossref  = {DBLP:conf/nips/2015},
  timestamp = {Fri, 08 Apr 2016 19:32:52 +0200}
}



@inproceedings{DBLP:conf/iccv/MaoLXLWS17,
  author    = {Xudong Mao and
               Qing Li and
               Haoran Xie and
               Raymond Y. K. Lau and
               Zhen Wang and
               Stephen Paul Smolley},
  title     = {Least Squares Generative Adversarial Networks},
  booktitle = {{IEEE} International Conference on Computer Vision, {ICCV} 2017, Venice,
               Italy, October 22-29, 2017},
  pages     = {2813--2821},
  year      = {2017},
  crossref  = {DBLP:conf/iccv/2017},
  timestamp = {Fri, 02 Nov 2018 09:49:35 +0100},
}



@inproceedings{DBLP:conf/iccv/ChenK17,
  author    = {Qifeng Chen and
               Vladlen Koltun},
  title     = {Photographic Image Synthesis with Cascaded Refinement Networks},
  booktitle = {{IEEE} International Conference on Computer Vision, {ICCV} 2017, Venice,
               Italy, October 22-29, 2017},
  pages     = {1520--1529},
  year      = {2017},
  crossref  = {DBLP:conf/iccv/2017},
  timestamp = {Fri, 02 Nov 2018 09:49:36 +0100},
}


@inproceedings{DBLP:conf/iccv/ZhangXL17,
  author    = {Han Zhang and
               Tao Xu and
               Hongsheng Li},
  title     = {StackGAN: Text to Photo-Realistic Image Synthesis with Stacked Generative
               Adversarial Networks},
  booktitle = {{IEEE} International Conference on Computer Vision, {ICCV} 2017, Venice,
               Italy, October 22-29, 2017},
  pages     = {5908--5916},
  year      = {2017},
  crossref  = {DBLP:conf/iccv/2017},
  timestamp = {Thu, 11 Jan 2018 13:21:37 +0100},
}

@inproceedings{DBLP:conf/nips/HeuselRUNH17,
  author    = {Martin Heusel and
               Hubert Ramsauer and
               Thomas Unterthiner and
               Bernhard Nessler and
               Sepp Hochreiter},
  title     = {GANs Trained by a Two Time-Scale Update Rule Converge to a Local Nash
               Equilibrium},
  booktitle = {Advances in Neural Information Processing Systems 30: Annual Conference
               on Neural Information Processing Systems 2017, 4-9 December 2017,
               Long Beach, CA, {USA}},
  pages     = {6629--6640},
  year      = {2017},
  crossref  = {DBLP:conf/nips/2017},
  timestamp = {Mon, 27 Nov 2017 12:38:48 +0100},
}

@InProceedings{Schroff2015,
  author    = {Florian Schroff and Dmitry Kalenichenko and James Philbin},
  title     = {FaceNet: {A} unified embedding for face recognition and clustering},
  booktitle = {{IEEE} Conference on Computer Vision and Pattern Recognition, {CVPR} 2015, Boston, MA, USA, June 7-12, 2015},
  year      = {2015},
  pages     = {815--823},
  crossref  = {DBLP:conf/cvpr/2015},
  timestamp = {Thu, 25 May 2017 00:41:13 +0200},
}

@inproceedings{DBLP:conf/nips/GoodfellowPMXWOCB14,
  author    = {Ian J. Goodfellow and
               Jean Pouget{-}Abadie and
               Mehdi Mirza and
               Bing Xu and
               David Warde{-}Farley and
               Sherjil Ozair and
               Aaron C. Courville and
               Yoshua Bengio},
  title     = {Generative Adversarial Nets},
  booktitle = {Advances in Neural Information Processing Systems 27: Annual Conference
               on Neural Information Processing Systems 2014, December 8-13 2014,
               Montreal, Quebec, Canada},
  pages     = {2672--2680},
  year      = {2014},
  crossref  = {DBLP:conf/nips/2014},
  timestamp = {Wed, 10 Dec 2014 21:34:12 +0100},
}

@inproceedings{DBLP:conf/nips/vid2vid,
  author    = {Ting{-}Chun Wang and
               Ming{-}Yu Liu and
               Jun{-}Yan Zhu and
               Nikolai Yakovenko and
               Andrew Tao and
               Jan Kautz and
               Bryan Catanzaro},
  title     = {Video-to-Video Synthesis},
  booktitle = {Advances in Neural Information Processing Systems 31: Annual Conference
               on Neural Information Processing Systems 2018, NeurIPS 2018, 3-8 December
               2018, Montr{\'{e}}al, Canada.},
  pages     = {1152--1164},
  year      = {2018},
  crossref  = {DBLP:conf/nips/2018},
  timestamp = {Sun, 16 Dec 2018 17:30:05 +0100},
}

@inproceedings{DBLP:conf/avss/BochinskiES17,
  author    = {Erik Bochinski and
               Volker Eiselein and
               Thomas Sikora},
  title     = {High-Speed tracking-by-detection without using image information},
  booktitle = {14th {IEEE} International Conference on Advanced Video and Signal
               Based Surveillance, {AVSS} 2017, Lecce, Italy, August 29 - September
               1, 2017},
  pages     = {1--6},
  year      = {2017},
  crossref  = {DBLP:conf/avss/2017},
  timestamp = {Mon, 19 Feb 2018 16:01:50 +0100},
}


@inproceedings{DBLP:conf/eccv/RenLR18,
  author    = {Zhongzheng Ren and
               Yong Jae Lee and
               Michael S. Ryoo},
  title     = {Learning to Anonymize Faces for Privacy Preserving Action Detection},
  booktitle = {Computer Vision - {ECCV} 2018 - 15th European Conference, Munich,
               Germany, September 8-14, 2018, Proceedings, Part {I}},
  pages     = {639--655},
  year      = {2018},
  crossref  = {DBLP:conf/eccv/2018-1},
  timestamp = {Tue, 14 May 2019 10:00:45 +0200},
}

@inproceedings{DBLP:conf/cvpr/ShiraiW19,
  author    = {Sola Shirai and
               Jacob Whitehill},
  title     = {Privacy-Preserving Annotation of Face Images Through Attribute-Preserving
               Face Synthesis},
  booktitle = {{IEEE} Conference on Computer Vision and Pattern Recognition Workshops,
               {CVPR} Workshops 2019, Long Beach, CA, USA, June 16-20, 2019},
  year      = {2019},
  crossref  = {DBLP:conf/cvpr/2019w},
  timestamp = {Wed, 18 Dec 2019 15:22:07 +0100},
}

@InProceedings{DBLP:conf/cvpr/Yeh0LSHD17,
  author    = {Raymond A. Yeh and Chen Chen and Teck{-}Yian Lim and Alexander G. Schwing and Mark Hasegawa{-}Johnson and Minh N. Do},
  title     = {Semantic Image Inpainting with Deep Generative Models},
  booktitle = {2017 {IEEE} Conference on Computer Vision and Pattern Recognition, {CVPR} 2017, Honolulu, HI, USA, July 21-26, 2017},
  year      = {2017},
  pages     = {6882--6890},
  crossref  = {DBLP:conf/cvpr/2017},
  file      = {:/home/pblies/literature/gans/Semantic Image Inpainting with Deep Generative Models.pdf:PDF},
  timestamp = {Wed, 16 Oct 2019 14:14:50 +0200},
}
@ARTICLE{Figueredo:2009dg,
   author = {Figueredo, A.~J. and Wolf, P. S.~A.},
   title = {Assortative pairing and life history strategy - a cross-cultural study.},
   journal = {Human Nature},
   volume = {20},
   pages = {317-330},
   year = {2009}
}

@InProceedings{Hu_2017_CVPR,
author = {Hu, Peiyun and Ramanan, Deva},
title = {Finding Tiny Faces},
booktitle = {The IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
month = {July},
year = {2017}
} 

@article{DBLP:journals/corr/ZhangZL016,
  author    = {Kaipeng Zhang and
               Zhanpeng Zhang and
               Zhifeng Li and
               Yu Qiao},
  title     = {Joint Face Detection and Alignment using Multi-task Cascaded Convolutional
               Networks},
  journal   = {CoRR},
  volume    = {abs/1604.02878},
  year      = {2016},
  archivePrefix = {arXiv},
  eprint    = {1604.02878},
  timestamp = {Mon, 13 Aug 2018 16:46:42 +0200},
}



@article{DBLP:journals/corr/ArjovskyCB17,
       author = {{Arjovsky}, Martin and {Chintala}, Soumith and {Bottou}, L{\'e}on},
        title = "{Wasserstein GAN}",
      journal = {arXiv e-prints},
     keywords = {Statistics - Machine Learning, Computer Science - Machine Learning},
         year = 2017,
        month = jan,
          eid = {arXiv:1701.07875},
        pages = {arXiv:1701.07875},
archivePrefix = {arXiv},
       eprint = {1701.07875},
 primaryClass = {stat.ML},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017arXiv170107875A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{DBLP:journals/corr/abs-1805-08318,
  author    = {Han Zhang and
               Ian J. Goodfellow and
               Dimitris N. Metaxas and
               Augustus Odena},
  title     = {Self-Attention Generative Adversarial Networks},
  journal   = {CoRR},
  volume    = {abs/1805.08318},
  year      = {2018},
  archivePrefix = {arXiv},
  eprint    = {1805.08318},
  timestamp = {Mon, 13 Aug 2018 16:47:52 +0200},
}

@incollection{Burt:1987:LPC:33517.33571,
 author = {Burt, Peter J. and Adelson, Edward H.},
 chapter = {The Laplacian Pyramid As a Compact Image Code},
 title = {Readings in Computer Vision: Issues, Problems, Principles, and Paradigms},
 editor = {Fischler, Martin A. and Firschein, Oscar},
 year = {1987},
 isbn = {0-934613-33-8},
 pages = {671--679},
 numpages = {9},
 acmid = {33571},
 publisher = {Morgan Kaufmann Publishers Inc.},
 address = {San Francisco, CA, USA},
} 

@InProceedings{DBLP:conf/cvpr/HuangLPHB17,
  author    = {Xun Huang and Yixuan Li and Omid Poursaeed and John E. Hopcroft and Serge J. Belongie},
  title     = {Stacked Generative Adversarial Networks},
  booktitle = {2017 {IEEE} Conference on Computer Vision and Pattern Recognition, {CVPR} 2017, Honolulu, HI, USA, July 21-26, 2017},
  year      = {2017},
  pages     = {1866--1875},
  timestamp = {Tue, 14 Nov 2017 17:15:06 +0100},
}

@article{DBLP:journals/corr/abs-1802-05957,
       author = {{Miyato}, Takeru and {Kataoka}, Toshiki and {Koyama}, Masanori and
         {Yoshida}, Yuichi},
        title = "{Spectral Normalization for Generative Adversarial Networks}",
      journal = {arXiv e-prints},
     keywords = {Computer Science - Machine Learning, Computer Science - Computer Vision and Pattern Recognition, Statistics - Machine Learning},
         year = 2018,
        month = feb,
          eid = {arXiv:1802.05957},
        pages = {arXiv:1802.05957},
archivePrefix = {arXiv},
       eprint = {1802.05957},
 primaryClass = {cs.LG},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018arXiv180205957M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@article{DBLP:journals/corr/TheisOB15,
  author    = {Lucas Theis and
               A{\"{a}}ron van den Oord and
               Matthias Bethge},
  title     = {A note on the evaluation of generative models},
  journal   = {CoRR},
  volume    = {abs/1511.01844},
  year      = {2015},
  archivePrefix = {arXiv},
  eprint    = {1511.01844},
  timestamp = {Mon, 13 Aug 2018 16:48:39 +0200},
}

@article{DBLP:journals/corr/TranRB17,
       author = {{Tran}, Dustin and {Ranganath}, Rajesh and {Blei}, David M.},
        title = "{Hierarchical Implicit Models and Likelihood-Free Variational Inference}",
      journal = {arXiv e-prints},
     keywords = {Statistics - Machine Learning, Computer Science - Machine Learning, Statistics - Computation, Statistics - Methodology},
         year = 2017,
        month = feb,
          eid = {arXiv:1702.08896},
        pages = {arXiv:1702.08896},
archivePrefix = {arXiv},
       eprint = {1702.08896},
 primaryClass = {stat.ML},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017arXiv170208896T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@misc{IOUTracker,
  title = {IOU Tracker},
  howpublished = {\url{https://github.com/bochinski/iou-tracker}}},
  note = {Accessed: 2018-12-19}
}


@article{fvd,
       author = {{Unterthiner}, Thomas and {van Steenkiste}, Sjoerd and {Kurach}, Karol
        and {Marinier}, Raphael and {Michalski}, Marcin and {Gelly},
        Sylvain},
        title = "{Towards Accurate Generative Models of Video: A New Metric \&
        Challenges}",
      journal = {arXiv e-prints},
     keywords = {Computer Science - Computer Vision and Pattern Recognition, Computer
        Science - Artificial Intelligence, Computer Science - Machine
        Learning, Computer Science - Neural and Evolutionary Computing,
        Statistics - Machine Learning},
         year = 2018,
        month = Dec,
          eid = {arXiv:1812.01717},
        pages = {arXiv:1812.01717},
archivePrefix = {arXiv},
       eprint = {1812.01717},
 primaryClass = {cs.CV},
       adsurl = {https://ui.adsabs.harvard.edu/\#abs/2018arXiv181201717U},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@InProceedings{DBLP:conf/isvc/HukkelasML19,
  author    = {Hukkel{\aa}s, H{\aa}kon and Mester, Rudolf and Lindseth, Frank},
  title     = {DeepPrivacy: A Generative Adversarial Network for Face Anonymization},
  booktitle = {Advances in Visual Computing},
  year      = {2019},
  editor    = {Bebis, George and Boyle, Richard and Parvin, Bahram and Koracin, Darko and Ushizima, Daniela and Chai, Sek and Sueda, Shinjiro and Lin, Xin and Lu, Aidong and Thalmann, Daniel and Wang, Chaoli and Xu, Panpan},
  pages     = {565--578},
  address   = {Cham},
  publisher = {Springer International Publishing},
  file      = {:/home/pblies/literature/gans/DeepPrivacy  A Generative Adversarial Networkfor Face Anonymization.pdf:PDF},
  isbn      = {978-3-030-33720-9},
}

@InProceedings{ganonymizer,
  author    = {Tanimura, Tomoki and Kawano, Makoto and Yonezawa, Takuro and Nakazawa, Jin},
  title     = {GANonymizer: Image Anonymization Method Integrating Object Detection and Generative Adversarial Network},
  booktitle = {3rd EAI International Conference on IoT in Urban Space},
  year      = {2020},
  editor    = {Jos{\'e}, Rui and Van Laerhoven, Kristof and Rodrigues, Helena},
  pages     = {109--121},
  address   = {Cham},
  publisher = {Springer International Publishing},
  file      = {:/home/pblies/literature/gans/ganonymizer_urbiot2018.pdf:PDF},
  isbn      = {978-3-030-28925-6},
}

@misc{dHash,
  author= {Neal Krawetz},
  title = {},
  howpublished = {\url{http://www.hackerfactor.com/blog/?/archives/529-Kind-of-Like-That.html}}}
}


@proceedings{DBLP:conf/avss/2017,
  title     = {14th {IEEE} International Conference on Advanced Video and Signal
               Based Surveillance, {AVSS} 2017, Lecce, Italy, August 29 - September
               1, 2017},
  publisher = {{IEEE}},
  year      = {2017},
  ntIssue.jsp?punumber=8055736},
  isbn      = {978-1-5386-2939-0},
  timestamp = {Fri, 27 Oct 2017 12:27:12 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/avss/2017},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{stngan,
author = {Wu, Yifan and Singh, Vivek and Kapoor, Ankur},
year = {2019},
month = {11},
pages = {},
title = {From Image to Video Face Inpainting: Spatial-Temporal Nested GAN (STN-GAN) for Usability Recovery}
}

@proceedings{DBLP:conf/cvpr/2019w,
  title     = {{IEEE} Conference on Computer Vision and Pattern Recognition Workshops,
               {CVPR} Workshops 2019, Long Beach, CA, USA, June 16-20, 2019},
  publisher = {Computer Vision Foundation / {IEEE}},
  year      = {2019},
  timestamp = {Wed, 18 Dec 2019 15:22:07 +0100},
  biburl    = {https://dblp.org/rec/bib/conf/cvpr/2019w},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


@proceedings{DBLP:conf/nips/2018,
  editor    = {Samy Bengio and
               Hanna M. Wallach and
               Hugo Larochelle and
               Kristen Grauman and
               Nicol{\`{o}} Cesa{-}Bianchi and
               Roman Garnett},
  title     = {Advances in Neural Information Processing Systems 31: Annual Conference
               on Neural Information Processing Systems 2018, NeurIPS 2018, 3-8 December
               2018, Montr{\'{e}}al, Canada},
  year      = {2018},
  timestamp = {Sun, 16 Dec 2018 17:30:05 +0100},
}

@proceedings{DBLP:conf/eccv/2018-1,
  editor    = {Vittorio Ferrari and
               Martial Hebert and
               Cristian Sminchisescu and
               Yair Weiss},
  title     = {Computer Vision - {ECCV} 2018 - 15th European Conference, Munich,
               Germany, September 8-14, 2018, Proceedings, Part {I}},
  series    = {Lecture Notes in Computer Science},
  volume    = {11205},
  publisher = {Springer},
  year      = {2018},
  isbn      = {978-3-030-01245-8},
  timestamp = {Tue, 14 May 2019 10:00:45 +0200},
}

@proceedings{DBLP:conf/eccv/2018-14,
  editor    = {Vittorio Ferrari and
               Martial Hebert and
               Cristian Sminchisescu and
               Yair Weiss},
  title     = {Computer Vision - {ECCV} 2018 - 15th European Conference, Munich,
               Germany, September 8-14, 2018, Proceedings, Part {XIV}},
  series    = {Lecture Notes in Computer Science},
  volume    = {11218},
  publisher = {Springer},
  year      = {2018},
  isbn      = {978-3-030-01263-2},
  timestamp = {Tue, 14 May 2019 10:00:45 +0200},
}

@proceedings{DBLP:conf/icmcs/2019,
  title     = {{IEEE} International Conference on Multimedia and Expo, {ICME} 2019,
               Shanghai, China, July 8-12, 2019},
  publisher = {{IEEE}},
  year      = {2019},
  isbn      = {978-1-5386-9552-4},
  timestamp = {Wed, 16 Oct 2019 14:14:56 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/icmcs/2019},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


@proceedings{DBLP:conf/nips/2014,
  editor    = {Zoubin Ghahramani and
               Max Welling and
               Corinna Cortes and
               Neil D. Lawrence and
               Kilian Q. Weinberger},
  title     = {Advances in Neural Information Processing Systems 27: Annual Conference
               on Neural Information Processing Systems 2014, December 8-13 2014,
               Montreal, Quebec, Canada},
  year      = {2014},
  timestamp = {Wed, 10 Dec 2014 21:34:12 +0100},
}



@proceedings{DBLP:conf/cvpr/2015,
  title     = {{IEEE} Conference on Computer Vision and Pattern Recognition, {CVPR}
               2015, Boston, MA, USA, June 7-12, 2015},
  publisher = {{IEEE} Computer Society},
  year      = {2015},
  isbn      = {978-1-4673-6964-0},
  timestamp = {Thu, 28 Apr 2016 10:52:27 +0200},
}



@proceedings{DBLP:conf/nips/2015,
  editor    = {Corinna Cortes and
               Neil D. Lawrence and
               Daniel D. Lee and
               Masashi Sugiyama and
               Roman Garnett},
  title     = {Advances in Neural Information Processing Systems 28: Annual Conference
               on Neural Information Processing Systems 2015, December 7-12, 2015,
               Montreal, Quebec, Canada},
  year      = {2015},
  timestamp = {Fri, 08 Apr 2016 19:32:52 +0200},
}

@proceedings{DBLP:conf/miccai/2015-3,
  editor    = {Nassir Navab and
               Joachim Hornegger and
               William M. Wells III and
               Alejandro F. Frangi},
  title     = {Medical Image Computing and Computer-Assisted Intervention - {MICCAI}
               2015 - 18th International Conference Munich, Germany, October 5 -
               9, 2015, Proceedings, Part {III}},
  series    = {Lecture Notes in Computer Science},
  volume    = {9351},
  publisher = {Springer},
  year      = {2015},
  isbn      = {978-3-319-24573-7},
  timestamp = {Tue, 23 May 2017 01:11:14 +0200},
}

@proceedings{DBLP:conf/iccv/2017,
  title     = {{IEEE} International Conference on Computer Vision, {ICCV} 2017, Venice,
               Italy, October 22-29, 2017},
  publisher = {{IEEE} Computer Society},
  year      = {2017},
  isbn      = {978-1-5386-1032-9},
  timestamp = {Thu, 11 Jan 2018 13:21:37 +0100},
}

@Proceedings{DBLP:conf/cvpr/2017,
  title     = {2017 {IEEE} Conference on Computer Vision and Pattern Recognition, {CVPR} 2017, Honolulu, HI, USA, July 21-26, 2017},
  year      = {2017},
  publisher = {{IEEE} Computer Society},
  isbn      = {978-1-5386-0457-1},
  timestamp = {Tue, 14 Nov 2017 09:55:57 +0100}
}

@proceedings{DBLP:conf/cvpr/2018,
  title     = {2018 {IEEE} Conference on Computer Vision and Pattern Recognition,
               {CVPR} 2018, Salt Lake City, UT, USA, June 18-22, 2018},
  publisher = {{IEEE} Computer Society},
  year      = {2018},
  timestamp = {Tue, 20 Nov 2018 12:25:14 +0100},
}

@proceedings{DBLP:conf/nips/2017,
  editor    = {Isabelle Guyon and
               Ulrike von Luxburg and
               Samy Bengio and
               Hanna M. Wallach and
               Rob Fergus and
               S. V. N. Vishwanathan and
               Roman Garnett},
  title     = {Advances in Neural Information Processing Systems 30: Annual Conference
               on Neural Information Processing Systems 2017, 4-9 December 2017,
               Long Beach, CA, {USA}},
  year      = {2017},
  timestamp = {Mon, 27 Nov 2017 12:38:16 +0100},
}


@proceedings{DBLP:conf/icml/2018,
  editor    = {Jennifer G. Dy and
               Andreas Krause},
  title     = {Proceedings of the 35th International Conference on Machine Learning,
               {ICML} 2018, Stockholmsm{\"{a}}ssan, Stockholm, Sweden, July
               10-15, 2018},
  series    = {{JMLR} Workshop and Conference Proceedings},
  volume    = {80},
  publisher = {JMLR.org},
  year      = {2018},
  timestamp = {Fri, 13 Jul 2018 14:57:00 +0200},
}

@InProceedings{DBLP:conf/cvpr/LiLY017,
  author    = {Yijun Li and Sifei Liu and Jimei Yang and Ming{-}Hsuan Yang},
  title     = {Generative Face Completion},
  booktitle = {2017 {IEEE} Conference on Computer Vision and Pattern Recognition, {CVPR} 2017, Honolulu, HI, USA, July 21-26, 2017},
  year      = {2017},
  pages     = {5892--5900},
  file      = {:/home/pblies/literature/gans/Generative Face Completion.pdf:PDF},
  timestamp = {Wed, 16 Oct 2019 14:14:50 +0200},
}


@InProceedings{DBLP:conf/cvpr/LiWWTQYWLH19,
  author    = {Jian Li and Yabiao Wang and Changan Wang and Ying Tai and Jianjun Qian and Jian Yang and Chengjie Wang and Jilin Li and Feiyue Huang},
  title     = {{DSFD:} Dual Shot Face Detector},
  booktitle = {{IEEE} Conference on Computer Vision and Pattern Recognition, {CVPR} 2019, Long Beach, CA, USA, June 16-20, 2019},
  year      = {2019},
  pages     = {5060--5069},
  crossref  = {DBLP:conf/cvpr/2019},
  file      = {:/home/pblies/literature/vision/Li_DSFD_Dual_Shot_Face_Detector_CVPR_2019_paper.pdf:PDF},
  timestamp = {Wed, 18 Dec 2019 15:22:07 +0100},
}

@inproceedings{DBLP:journals/corr/KingmaB14,
  author    = {Diederik P. Kingma and
               Jimmy Ba},
  editor    = {Yoshua Bengio and
               Yann LeCun},
  title     = {Adam: {A} Method for Stochastic Optimization},
  booktitle = {3rd International Conference on Learning Representations, {ICLR} 2015,
               San Diego, CA, USA, May 7-9, 2015, Conference Track Proceedings},
  year      = {2015},
  timestamp = {Thu, 25 Jul 2019 14:25:37 +0200},
}

